InterpNET: Neural Introspection for Interpretable Deep Learning

Humans are able to explain their reasoning. On the contrary, deep neural networks are not. This paper attempts to bridge this gap by introducing a new way to design interpretable neural networks for classification, inspired by physiological evidence of the human visual system's inner-workings. This paper proposes a neural network design paradigm, termed InterpNET, which can be combined with any existing classification architecture to generate natural language explanations of the classifications. The success of the module relies on the assumption that the network's computation and reasoning is represented in its internal layer activations. While in principle InterpNET could be applied to any existing classification architecture, it is evaluated via an image classification and explanation task. Experiments on a CUB bird classification and explanation dataset show qualitatively and quantitatively that the model is able to generate high-quality explanations. While the current state-of-the-art METEOR score on this dataset is 29.2, InterpNET achieves a much higher METEOR score of 37.9.

==> figures/beamwidth.tex <==
% This file was created by matplotlib2tikz v0.6.7.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.203921568627451,0.541176470588235,0.741176470588235}

\begin{axis}[
xlabel={beam width},
ylabel={BLEU Score},
xmin=0.45, xmax=12.55,
ymin=50.8238187064595, ymax=52.4259836085523,
ytick={50.8,51,51.2,51.4,51.6,51.8,52,52.2,52.4,52.6},
yticklabels={,51.0,51.2,51.4,51.6,51.8,52.0,52.2,52.4,},
tick align=outside,
tick pos=left,
xmajorgrids,
x grid style={lightgray!92.026143790849673!black},
ymajorgrids,
y grid style={lightgray!92.026143790849673!black},
axis line style={lightgray!98.300653594771248!black},
axis background/.style={fill=white!93.333333333333329!black}
]
\addplot [color0]
table {%
1 50.8966443838274
2 52.3531579311845
3 52.119771774103
4 52.0049724696058
5 52.0144679629864
6 52.0090319609503
7 51.9237396980346
8 51.8816711771832
9 51.9651279459875
10 51.9651279459875
11 51.9651279459875
12 51.9781077482748
};
\end{axis}

\end{tikzpicture}
